Improving neutrino energy estimation of charged-current interaction events with recurrent neural networks in MicroBooNE

We present a deep learning-based method for estimating the neutrino energy of charged-current neutrino-argon interactions. We employ a recurrent neural network (RNN) architecture for neutrino energy estimation in the MicroBooNE experiment, utilizing liquid argon time projection chamber (LArTPC) detector technology. Traditional energy estimation approaches in LArTPCs, which largely rely on reconstructing and summing visible energies, often experience sizable biases and resolution smearing because of the complex nature of neutrino interactions and the detector response. The estimation of neutrino energy can be improved after considering the kinematics information of reconstructed final-state particles. Utilizing kinematic information of reconstructed particles, the deep learning-based approach shows improved resolution and reduced bias for the muon neutrino Monte Carlo simulation sample compared to the traditional approach. In order to address the common concern about the effectiveness of this method on experimental data, the RNN-based energy estimator is further examined and validated with dedicated data-simulation consistency tests using MicroBooNE data. We also assess its potential impact on a neutrino oscillation study after accounting for all statistical and systematic uncertainties and show that it enhances physics sensitivity. This method has good potential to improve the performance of other physics analyses.

==> src/arch.tex <==
\begin{tikzpicture}[font=\fontsize{10}{10}\selectfont]]
  \tikzstyle{input PF}   = [circle, fill=colorInput, draw, minimum size=2.5em]
  \tikzstyle{preproc}    = [
    fill=colorPreproc, rotate=90, inner sep=0.6em, draw
  ]
  \tikzstyle{rnn}        = [
    regular polygon, regular polygon sides=4, fill=colorRNN, inner sep=-0.1em,
    draw
  ]

  \foreach \i/\x in {1/0, 2/2, N/5}
  {
    \node[input PF] (p\i)   at (\x, 0) {$P_\i$};
    \node[preproc, anchor=west] (pre\i) at ([yshift=1em]p\i.north) {Preproc};
    \node[rnn, anchor=south]    (rnn\i) at ([yshift=1em]pre\i.east) {RNN};

    \draw[gray, thick, ->] (p\i.north) -- (pre\i.west);
    \draw[gray, thick, ->] (pre\i.east) -- (rnn\i.south);
  }

  \foreach \i/\j in {1/2, 2/N}
  {
    \draw[gray, thick, ->] (rnn\i.east) -- (rnn\j.west);
  }

  \node (ddots) at ($(pre2)!0.5!(preN)$) {\huge \ldots};

  \tikzstyle{input event} = [circle, fill=colorEventNode, draw, inner sep=0.2em];
  \node[input event, anchor=south east] (event)
    at ([yshift=30pt]rnn1.north east) {Event};

  \tikzstyle{predict} = [fill=colorPredict, anchor=west, inner sep=1.0em, draw]
  \tikzstyle{output} = [circle, fill=colorOutput, anchor=west, inner sep=0.3em, draw]

  \node[predict, anchor=west] (predict)
    at ([xshift=50pt]rnnN.east) {Predictor};
  \node[output]  (output)  [right=of predict] {Energy};

  \draw[gray, thick, ->] (predict.east) -- (output.west);

  \tikzstyle{concat} = [circle, inner sep=0]
  \node[concat] (concat) at ($(rnnN.east)!0.5!(predict.west)$)
    {\Large $\oplus$};

  \draw[gray, thick, ->] (rnnN.east) -- (concat.west);
  \draw[gray, thick, ->] (event.east) -- (concat |- event) -- (concat.north);
  \draw[gray, thick, ->] (concat.east) -- (predict.west);

  \tikzstyle{legend} = [ rectangle, rounded corners, draw, inner sep=0.3em ]
  \tikzstyle{layer} = [
    rectangle, rounded corners, text=black, fill=colorLayer,
    anchor=north, draw
  ]

  \node[legend, anchor=north east, fill=colorLegend] (legend)
    at (output.east |- pre1.east)
  {
    \begin{tikzpicture}
      \node[layer] (norm)  at (0, 0) {\texttt{BatchNorm}};

      \node[rectangle, anchor=south] (title) at ([yshift=5pt]norm.north)
        {Preproc \& Predictor};

      \node[legend, anchor=north, fill=colorBlock] (MLPBlock)
        at ([yshift=-3pt]norm.south)
      {
        \begin{tikzpicture}
          \node[layer] (fc)   at (0, 0) {\texttt{Dense(128)}};
          \node[layer] (norm) at ([yshift=-3pt] fc.south) {\texttt{BatchNorm}};
        \end{tikzpicture}
      };

      \node[circle, anchor=north west, color=black] (x3)
        at (MLPBlock.north east) {$\times 3$};
    \end{tikzpicture}
  };

  \node[legend, anchor=east, font=\small] (legendIO)
    at (output.east |- event.east)
  {
    \begin{tikzpicture}
    \node[concat] (concat) at (0, 0) {\Large $\oplus$};
    \node[anchor=west] (eventLabel) at ([xshift=3pt] concat.east)
      {Concatenation};
    \end{tikzpicture}
  };

\end{tikzpicture}



==> src/authors/microboone-author-list-december2022-PRD.tex <==

\newcommand{\ANL}{Argonne National Laboratory (ANL), Lemont, IL, 60439, USA}
\newcommand{\Bern}{Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\newcommand{\BNL}{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\newcommand{\UCSB}{University of California, Santa Barbara, CA, 93106, USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\CIEMAT}{Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid E-28040, Spain}
\newcommand{\Chicago}{University of Chicago, Chicago, IL, 60637, USA}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, 45221, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, 80523, USA}
\newcommand{\Columbia}{Columbia University, New York, NY, 10027, USA}
\newcommand{\Edinburgh}{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\newcommand{\Granada}{Universidad de Granada, Granada E-18071, Spain}
\newcommand{\Harvard}{Harvard University, Cambridge, MA 02138, USA}
\newcommand{\IIT}{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\newcommand{\KSU}{Kansas State University (KSU), Manhattan, KS, 66506, USA}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\newcommand{\Louisiana}{Louisiana State University, Baton Rouge, LA, 70803, USA}
\newcommand{\Manchester}{The University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\MIT}{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\newcommand{\Michigan}{University of Michigan, Ann Arbor, MI, 48109, USA}
\newcommand{\Minnesota}{University of Minnesota, Minneapolis, MN, 55455, USA}
\newcommand{\NMSU}{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\newcommand{\Oxford}{University of Oxford, Oxford OX1 3RH, United Kingdom}
\newcommand{\Pitt}{University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, 08854, USA}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology (SDSMT), Rapid City, SD, 57701, USA}
\newcommand{\Maine}{University of Southern Maine, Portland, ME, 04104, USA}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY, 13244, USA}
\newcommand{\TelAviv}{Tel Aviv University, Tel Aviv, Israel, 69978}
\newcommand{\Tennessee}{University of Tennessee, Knoxville, TN, 37996, USA}
\newcommand{\UTA}{University of Texas, Arlington, TX, 76019, USA}
\newcommand{\Tufts}{Tufts University, Medford, MA, 02155, USA}
\newcommand{\UCL}{University College London, London WC1E 6BT, United Kingdom}
\newcommand{\VTech}{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\newcommand{\Warwick}{University of Warwick, Coventry CV4 7AL, United Kingdom}
\newcommand{\Yale}{Wright Laboratory, Department of Physics, Yale University, New Haven, CT, 06520, USA}

\affiliation{\ANL}
\affiliation{\Bern}
\affiliation{\BNL}
\affiliation{\UCSB}
\affiliation{\Cambridge}
\affiliation{\CIEMAT}
\affiliation{\Chicago}
\affiliation{\Cincinnati}
\affiliation{\CSU}
\affiliation{\Columbia}
\affiliation{\Edinburgh}
\affiliation{\FNAL}
\affiliation{\Granada}
\affiliation{\Harvard}
\affiliation{\IIT}
\affiliation{\KSU}
\affiliation{\Lancaster}
\affiliation{\LANL}
\affiliation{\Louisiana}
\affiliation{\Manchester}
\affiliation{\MIT}
\affiliation{\Michigan}
\affiliation{\Minnesota}
\affiliation{\NMSU}
\affiliation{\Oxford}
\affiliation{\Pitt}
\affiliation{\Rutgers}
\affiliation{\SLAC}
\affiliation{\SDSMT}
\affiliation{\Maine}
\affiliation{\Syracuse}
\affiliation{\TelAviv}
\affiliation{\Tennessee}
\affiliation{\UTA}
\affiliation{\Tufts}
\affiliation{\UCL}
\affiliation{\VTech}
\affiliation{\Warwick}
\affiliation{\Yale}

\author{P.~Abratenko} \affiliation{\Tufts}
\author{O.~Alterkait} \affiliation{\Tufts}
\author{D.~Andrade~Aldana} \affiliation{\IIT}
\author{J.~Anthony} \affiliation{\Cambridge}
\author{L.~Arellano} \affiliation{\Manchester}
\author{J.~Asaadi} \affiliation{\UTA}
\author{A.~Ashkenazi}\affiliation{\TelAviv}
\author{S.~Balasubramanian}\affiliation{\FNAL}
\author{B.~Baller} \affiliation{\FNAL}
\author{G.~Barr} \affiliation{\Oxford}
\author{J.~Barrow} \affiliation{\MIT}\affiliation{\TelAviv}
\author{V.~Basque} \affiliation{\FNAL}
\author{O.~Benevides~Rodrigues} \affiliation{\Syracuse}
\author{S.~Berkman} \affiliation{\FNAL}
\author{A.~Bhanderi} \affiliation{\Manchester}
\author{A.~Bhat} \affiliation{\Yale}
\author{M.~Bhattacharya} \affiliation{\FNAL}
\author{M.~Bishai} \affiliation{\BNL}
\author{A.~Blake} \affiliation{\Lancaster}
\author{B.~Bogart} \affiliation{\Michigan}
\author{T.~Bolton} \affiliation{\KSU}
\author{J.~Y.~Book} \affiliation{\Harvard}
\author{L.~Camilleri} \affiliation{\Columbia}
\author{Y.~Cao} \affiliation{\Manchester}
\author{D.~Caratelli} \affiliation{\UCSB}
\author{I.~Caro~Terrazas} \affiliation{\CSU}
\author{F.~Cavanna} \affiliation{\FNAL}
\author{G.~Cerati} \affiliation{\FNAL}
\author{Y.~Chen} \affiliation{\SLAC}
\author{J.~M.~Conrad} \affiliation{\MIT}
\author{M.~Convery} \affiliation{\SLAC}
\author{L.~Cooper-Troendle} \affiliation{\Yale}
\author{J.~I.~Crespo-Anad\'{o}n} \affiliation{\CIEMAT}
\author{M.~Del~Tutto} \affiliation{\FNAL}
\author{S.~R.~Dennis} \affiliation{\Cambridge}
\author{P.~Detje} \affiliation{\Cambridge}
\author{A.~Devitt} \affiliation{\Lancaster}
\author{R.~Diurba} \affiliation{\Bern}
\author{Z.~Djurcic} \affiliation{\ANL}
\author{R.~Dorrill} \affiliation{\IIT}
\author{K.~Duffy} \affiliation{\Oxford}
\author{S.~Dytman} \affiliation{\Pitt}
\author{B.~Eberly} \affiliation{\Maine}
\author{P.~Englezos} \affiliation{\Rutgers}
\author{A.~Ereditato} \affiliation{\Chicago}\affiliation{\FNAL}
\author{J.~J.~Evans} \affiliation{\Manchester}
\author{R.~Fine} \affiliation{\LANL}
\author{O.~G.~Finnerud} \affiliation{\Manchester}
\author{W.~Foreman} \affiliation{\IIT}
\author{B.~T.~Fleming} \affiliation{\Chicago}
\author{N.~Foppiani} \affiliation{\Harvard}
\author{D.~Franco} \affiliation{\Chicago}
\author{A.~P.~Furmanski}\affiliation{\Minnesota}
\author{D.~Garcia-Gamez} \affiliation{\Granada}
\author{S.~Gardiner} \affiliation{\FNAL}
\author{G.~Ge} \affiliation{\Columbia}
\author{S.~Gollapinni} \affiliation{\Tennessee}\affiliation{\LANL}
\author{O.~Goodwin} \affiliation{\Manchester}
\author{E.~Gramellini} \affiliation{\FNAL}
\author{P.~Green} \affiliation{\Manchester}\affiliation{\Oxford}
\author{H.~Greenlee} \affiliation{\FNAL}
\author{W.~Gu} \affiliation{\BNL}
\author{R.~Guenette} \affiliation{\Manchester}
\author{P.~Guzowski} \affiliation{\Manchester}
\author{L.~Hagaman} \affiliation{\Chicago}
\author{O.~Hen} \affiliation{\MIT}
\author{R.~Hicks} \affiliation{\LANL}
\author{C.~Hilgenberg}\affiliation{\Minnesota}
\author{G.~A.~Horton-Smith} \affiliation{\KSU}
\author{Z.~Imani} \affiliation{\Tufts}
\author{B.~Irwin} \affiliation{\Minnesota}
\author{R.~Itay} \affiliation{\SLAC}
\author{C.~James} \affiliation{\FNAL}
\author{X.~Ji} \affiliation{\BNL}
\author{L.~Jiang} \affiliation{\VTech}
\author{J.~H.~Jo} \affiliation{\BNL}\affiliation{\Yale}
\author{R.~A.~Johnson} \affiliation{\Cincinnati}
\author{Y.-J.~Jwa} \affiliation{\Columbia}
\author{D.~Kalra} \affiliation{\Columbia}
\author{N.~Kamp} \affiliation{\MIT}
\author{G.~Karagiorgi} \affiliation{\Columbia}
\author{W.~Ketchum} \affiliation{\FNAL}
\author{M.~Kirby} \affiliation{\FNAL}
\author{T.~Kobilarcik} \affiliation{\FNAL}
\author{I.~Kreslo} \affiliation{\Bern}
\author{M.~B.~Leibovitch} \affiliation{\UCSB}
\author{I.~Lepetic} \affiliation{\Rutgers}
\author{J.-Y. Li} \affiliation{\Edinburgh}
\author{K.~Li} \affiliation{\Yale}
\author{Y.~Li} \affiliation{\BNL}
\author{K.~Lin} \affiliation{\Rutgers}
\author{B.~R.~Littlejohn} \affiliation{\IIT}
\author{W.~C.~Louis} \affiliation{\LANL}
\author{X.~Luo} \affiliation{\UCSB}
\author{C.~Mariani} \affiliation{\VTech}
\author{D.~Marsden} \affiliation{\Manchester}
\author{J.~Marshall} \affiliation{\Warwick}
\author{N.~Martinez} \affiliation{\KSU}
\author{D.~A.~Martinez~Caicedo} \affiliation{\SDSMT}
\author{K.~Mason} \affiliation{\Tufts}
\author{A.~Mastbaum} \affiliation{\Rutgers}
\author{N.~McConkey} \affiliation{\Manchester}\affiliation{\UCL}
\author{V.~Meddage} \affiliation{\KSU}
\author{K.~Miller} \affiliation{\Chicago}
\author{J.~Mills} \affiliation{\Tufts}
\author{A.~Mogan} \affiliation{\CSU}
\author{T.~Mohayai} \affiliation{\FNAL}
\author{M.~Mooney} \affiliation{\CSU}
\author{A.~F.~Moor} \affiliation{\Cambridge}
\author{C.~D.~Moore} \affiliation{\FNAL}
\author{L.~Mora~Lepin} \affiliation{\Manchester}
\author{S.~Mulleriababu} \affiliation{\Bern}
\author{D.~Naples} \affiliation{\Pitt}
\author{A.~Navrer-Agasson} \affiliation{\Manchester}
\author{N.~Nayak} \affiliation{\BNL}
\author{M.~Nebot-Guinot}\affiliation{\Edinburgh}
\author{J.~Nowak} \affiliation{\Lancaster}
\author{N.~Oza} \affiliation{\Columbia}\affiliation{\LANL}
\author{O.~Palamara} \affiliation{\FNAL}
\author{N.~Pallat} \affiliation{\Minnesota}
\author{V.~Paolone} \affiliation{\Pitt}
\author{A.~Papadopoulou} \affiliation{\ANL}\affiliation{\MIT}
\author{V.~Papavassiliou} \affiliation{\NMSU}
\author{H.~B.~Parkinson} \affiliation{\Edinburgh}
\author{S.~F.~Pate} \affiliation{\NMSU}
\author{N.~Patel} \affiliation{\Lancaster}
\author{Z.~Pavlovic} \affiliation{\FNAL}
\author{E.~Piasetzky} \affiliation{\TelAviv}
\author{I.~D.~Ponce-Pinto} \affiliation{\Chicago}
\author{I.~Pophale} \affiliation{\Lancaster}
\author{S.~Prince} \affiliation{\Harvard}
\author{X.~Qian} \affiliation{\BNL}
\author{J.~L.~Raaf} \affiliation{\FNAL}
\author{V.~Radeka} \affiliation{\BNL}
\author{A.~Rafique} \affiliation{\ANL}
\author{M.~Reggiani-Guzzo} \affiliation{\Manchester}
\author{L.~Ren} \affiliation{\NMSU}
\author{L.~Rochester} \affiliation{\SLAC}
\author{J.~Rodriguez Rondon} \affiliation{\SDSMT}
\author{M.~Rosenberg} \affiliation{\Tufts}
\author{M.~Ross-Lonergan} \affiliation{\LANL}
\author{C.~Rudolf~von~Rohr} \affiliation{\Bern}
\author{G.~Scanavini} \affiliation{\Yale}
\author{D.~W.~Schmitz} \affiliation{\Chicago}
\author{A.~Schukraft} \affiliation{\FNAL}
\author{W.~Seligman} \affiliation{\Columbia}
\author{M.~H.~Shaevitz} \affiliation{\Columbia}
\author{R.~Sharankova} \affiliation{\FNAL}
\author{J.~Shi} \affiliation{\Cambridge}
\author{E.~L.~Snider} \affiliation{\FNAL}
\author{M.~Soderberg} \affiliation{\Syracuse}
\author{S.~S{\"o}ldner-Rembold} \affiliation{\Manchester}
\author{J.~Spitz} \affiliation{\Michigan}
\author{M.~Stancari} \affiliation{\FNAL}
\author{J.~St.~John} \affiliation{\FNAL}
\author{T.~Strauss} \affiliation{\FNAL}
\author{S.~Sword-Fehlberg} \affiliation{\NMSU}
\author{A.~M.~Szelc} \affiliation{\Edinburgh}
\author{W.~Tang} \affiliation{\Tennessee}
\author{N.~Taniuchi} \affiliation{\Cambridge}
\author{K.~Terao} \affiliation{\SLAC}
\author{C.~Thorpe} \affiliation{\Lancaster}
\author{D.~Torbunov} \affiliation{\BNL}
\author{D.~Totani} \affiliation{\UCSB}
\author{M.~Toups} \affiliation{\FNAL}
\author{Y.-T.~Tsai} \affiliation{\SLAC}
\author{J.~Tyler} \affiliation{\KSU}
\author{M.~A.~Uchida} \affiliation{\Cambridge}
\author{T.~Usher} \affiliation{\SLAC}
\author{B.~Viren} \affiliation{\BNL}
\author{M.~Weber} \affiliation{\Bern}
\author{H.~Wei} \affiliation{\Louisiana}
\author{A.~J.~White} \affiliation{\Chicago}
\author{Z.~Williams} \affiliation{\UTA}
\author{S.~Wolbers} \affiliation{\FNAL}
\author{T.~Wongjirad} \affiliation{\Tufts}
\author{M.~Wospakrik} \affiliation{\FNAL}
\author{K.~Wresilo} \affiliation{\Cambridge}
\author{N.~Wright} \affiliation{\MIT}
\author{W.~Wu} \affiliation{\FNAL}
\author{E.~Yandel} \affiliation{\UCSB}
\author{T.~Yang} \affiliation{\FNAL}
\author{L.~E.~Yates} \affiliation{\FNAL}
\author{H.~W.~Yu} \affiliation{\BNL}
\author{G.~P.~Zeller} \affiliation{\FNAL}
\author{J.~Zennamo} \affiliation{\FNAL}
\author{C.~Zhang} \affiliation{\BNL}

\collaboration{The MicroBooNE Collaboration}
\thanks{microboone\_info@fnal.gov}\noaffiliation


==> src/authors/microboone-author-list-may2023-PRD.tex <==


\newcommand{\ANL}{Argonne National Laboratory (ANL), Lemont, IL, 60439, USA}
\newcommand{\Bern}{Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\newcommand{\BNL}{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\newcommand{\UCSB}{University of California, Santa Barbara, CA, 93106, USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\CIEMAT}{Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid E-28040, Spain}
\newcommand{\Chicago}{University of Chicago, Chicago, IL, 60637, USA}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, 45221, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, 80523, USA}
\newcommand{\Columbia}{Columbia University, New York, NY, 10027, USA}
\newcommand{\Edinburgh}{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\newcommand{\Granada}{Universidad de Granada, Granada E-18071, Spain}
\newcommand{\Harvard}{Harvard University, Cambridge, MA 02138, USA}
\newcommand{\IIT}{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\newcommand{\KSU}{Kansas State University (KSU), Manhattan, KS, 66506, USA}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\newcommand{\Louisiana}{Louisiana State University, Baton Rouge, LA, 70803, USA}
\newcommand{\Manchester}{The University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\MIT}{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\newcommand{\Michigan}{University of Michigan, Ann Arbor, MI, 48109, USA}
\newcommand{\Minnesota}{University of Minnesota, Minneapolis, MN, 55455, USA}
\newcommand{\NMSU}{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\newcommand{\Oxford}{University of Oxford, Oxford OX1 3RH, United Kingdom}
\newcommand{\Pitt}{University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, 08854, USA}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology (SDSMT), Rapid City, SD, 57701, USA}
\newcommand{\Maine}{University of Southern Maine, Portland, ME, 04104, USA}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY, 13244, USA}
\newcommand{\TelAviv}{Tel Aviv University, Tel Aviv, Israel, 69978}
\newcommand{\Tennessee}{University of Tennessee, Knoxville, TN, 37996, USA}
\newcommand{\UTA}{University of Texas, Arlington, TX, 76019, USA}
\newcommand{\Tufts}{Tufts University, Medford, MA, 02155, USA}
\newcommand{\UCL}{University College London, London WC1E 6BT, United Kingdom}
\newcommand{\VTech}{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\newcommand{\Warwick}{University of Warwick, Coventry CV4 7AL, United Kingdom}
\newcommand{\Yale}{Wright Laboratory, Department of Physics, Yale University, New Haven, CT, 06520, USA}

\affiliation{\ANL}
\affiliation{\Bern}
\affiliation{\BNL}
\affiliation{\UCSB}
\affiliation{\Cambridge}
\affiliation{\CIEMAT}
\affiliation{\Chicago}
\affiliation{\Cincinnati}
\affiliation{\CSU}
\affiliation{\Columbia}
\affiliation{\Edinburgh}
\affiliation{\FNAL}
\affiliation{\Granada}
\affiliation{\Harvard}
\affiliation{\IIT}
\affiliation{\KSU}
\affiliation{\Lancaster}
\affiliation{\LANL}
\affiliation{\Louisiana}
\affiliation{\Manchester}
\affiliation{\MIT}
\affiliation{\Michigan}
\affiliation{\Minnesota}
\affiliation{\NMSU}
\affiliation{\Oxford}
\affiliation{\Pitt}
\affiliation{\Rutgers}
\affiliation{\SLAC}
\affiliation{\SDSMT}
\affiliation{\Maine}
\affiliation{\Syracuse}
\affiliation{\TelAviv}
\affiliation{\Tennessee}
\affiliation{\UTA}
\affiliation{\Tufts}
\affiliation{\UCL}
\affiliation{\VTech}
\affiliation{\Warwick}
\affiliation{\Yale}

\author{P.~Abratenko} \affiliation{\Tufts}
\author{O.~Alterkait} \affiliation{\Tufts}
\author{D.~Andrade~Aldana} \affiliation{\IIT}
\author{L.~Arellano} \affiliation{\Manchester}
\author{J.~Asaadi} \affiliation{\UTA}
\author{A.~Ashkenazi}\affiliation{\TelAviv}
\author{S.~Balasubramanian}\affiliation{\FNAL}
\author{B.~Baller} \affiliation{\FNAL}
\author{G.~Barr} \affiliation{\Oxford}
\author{D.~Barrow} \affiliation{\Oxford}
\author{J.~Barrow} \affiliation{\MIT}\affiliation{\TelAviv}
\author{V.~Basque} \affiliation{\FNAL}
\author{O.~Benevides~Rodrigues} \affiliation{\Syracuse}
\author{S.~Berkman} \affiliation{\FNAL}
\author{A.~Bhanderi} \affiliation{\Manchester}
\author{A.~Bhat} \affiliation{\Chicago}
\author{M.~Bhattacharya} \affiliation{\FNAL}
\author{M.~Bishai} \affiliation{\BNL}
\author{A.~Blake} \affiliation{\Lancaster}
\author{B.~Bogart} \affiliation{\Michigan}
\author{T.~Bolton} \affiliation{\KSU}
\author{J.~Y.~Book} \affiliation{\Harvard}
\author{L.~Camilleri} \affiliation{\Columbia}
\author{Y.~Cao} \affiliation{\Manchester}
\author{D.~Caratelli} \affiliation{\UCSB}
\author{I.~Caro~Terrazas} \affiliation{\CSU}
\author{F.~Cavanna} \affiliation{\FNAL}
\author{G.~Cerati} \affiliation{\FNAL}
\author{Y.~Chen} \affiliation{\SLAC}
\author{J.~M.~Conrad} \affiliation{\MIT}
\author{M.~Convery} \affiliation{\SLAC}
\author{L.~Cooper-Troendle} \affiliation{\Pitt}\affiliation{\Yale}
\author{J.~I.~Crespo-Anad\'{o}n} \affiliation{\CIEMAT}
\author{R.~Cross} \affiliation{\Warwick}
\author{M.~Del~Tutto} \affiliation{\FNAL}
\author{S.~R.~Dennis} \affiliation{\Cambridge}
\author{P.~Detje} \affiliation{\Cambridge}
\author{A.~Devitt} \affiliation{\Lancaster}
\author{R.~Diurba} \affiliation{\Bern}
\author{Z.~Djurcic} \affiliation{\ANL}
\author{R.~Dorrill} \affiliation{\IIT}
\author{K.~Duffy} \affiliation{\Oxford}
\author{S.~Dytman} \affiliation{\Pitt}
\author{B.~Eberly} \affiliation{\Maine}
\author{P.~Englezos} \affiliation{\Rutgers}
\author{A.~Ereditato} \affiliation{\Chicago}\affiliation{\FNAL}
\author{J.~J.~Evans} \affiliation{\Manchester}
\author{R.~Fine} \affiliation{\LANL}
\author{O.~G.~Finnerud} \affiliation{\Manchester}
\author{W.~Foreman} \affiliation{\IIT}
\author{B.~T.~Fleming} \affiliation{\Chicago}
\author{N.~Foppiani} \affiliation{\Harvard}
\author{D.~Franco} \affiliation{\Chicago}
\author{A.~P.~Furmanski}\affiliation{\Minnesota}
\author{D.~Garcia-Gamez} \affiliation{\Granada}
\author{S.~Gardiner} \affiliation{\FNAL}
\author{G.~Ge} \affiliation{\Columbia}
\author{S.~Gollapinni} \affiliation{\Tennessee}\affiliation{\LANL}
\author{O.~Goodwin} \affiliation{\Manchester}
\author{E.~Gramellini} \affiliation{\FNAL}
\author{P.~Green} \affiliation{\Oxford}
\author{H.~Greenlee} \affiliation{\FNAL}
\author{W.~Gu} \affiliation{\BNL}
\author{R.~Guenette} \affiliation{\Manchester}
\author{P.~Guzowski} \affiliation{\Manchester}
\author{L.~Hagaman} \affiliation{\Chicago}
\author{O.~Hen} \affiliation{\MIT}
\author{R.~Hicks} \affiliation{\LANL}
\author{C.~Hilgenberg}\affiliation{\Minnesota}
\author{G.~A.~Horton-Smith} \affiliation{\KSU}
\author{Z.~Imani} \affiliation{\Tufts}
\author{B.~Irwin} \affiliation{\Minnesota}
\author{R.~Itay} \affiliation{\SLAC}
\author{C.~James} \affiliation{\FNAL}
\author{X.~Ji} \affiliation{\BNL}
\author{L.~Jiang} \affiliation{\VTech}
\author{J.~H.~Jo} \affiliation{\BNL}
\author{R.~A.~Johnson} \affiliation{\Cincinnati}
\author{Y.-J.~Jwa} \affiliation{\Columbia}
\author{D.~Kalra} \affiliation{\Columbia}
\author{N.~Kamp} \affiliation{\MIT}
\author{G.~Karagiorgi} \affiliation{\Columbia}
\author{W.~Ketchum} \affiliation{\FNAL}
\author{M.~Kirby} \affiliation{\FNAL}
\author{T.~Kobilarcik} \affiliation{\FNAL}
\author{I.~Kreslo} \affiliation{\Bern}
\author{M.~B.~Leibovitch} \affiliation{\UCSB}
\author{I.~Lepetic} \affiliation{\Rutgers}
\author{J.-Y. Li} \affiliation{\Edinburgh}
\author{K.~Li} \affiliation{\Yale}
\author{Y.~Li} \affiliation{\BNL}
\author{K.~Lin} \affiliation{\Rutgers}
\author{B.~R.~Littlejohn} \affiliation{\IIT}
\author{H.~Liu} \affiliation{\BNL}
\author{W.~C.~Louis} \affiliation{\LANL}
\author{X.~Luo} \affiliation{\UCSB}
\author{C.~Mariani} \affiliation{\VTech}
\author{D.~Marsden} \affiliation{\Manchester}
\author{J.~Marshall} \affiliation{\Warwick}
\author{N.~Martinez} \affiliation{\KSU}
\author{D.~A.~Martinez~Caicedo} \affiliation{\SDSMT}
\author{S.~Martynenko} \affiliation{\BNL}
\author{A.~Mastbaum} \affiliation{\Rutgers}
\author{N.~McConkey} \affiliation{\UCL}
\author{V.~Meddage} \affiliation{\KSU}
\author{J.~Micallef} \affiliation{\MIT}\affiliation{\Tufts}
\author{K.~Miller} \affiliation{\Chicago}
\author{A.~Mogan} \affiliation{\CSU}
\author{T.~Mohayai} \affiliation{\FNAL}
\author{M.~Mooney} \affiliation{\CSU}
\author{A.~F.~Moor} \affiliation{\Cambridge}
\author{C.~D.~Moore} \affiliation{\FNAL}
\author{L.~Mora~Lepin} \affiliation{\Manchester}
\author{M.~Moudgalya} \affiliation{\Manchester}
\author{S.~Mulleriababu} \affiliation{\Bern}
\author{D.~Naples} \affiliation{\Pitt}
\author{A.~Navrer-Agasson} \affiliation{\Manchester}
\author{N.~Nayak} \affiliation{\BNL}
\author{M.~Nebot-Guinot}\affiliation{\Edinburgh}
\author{J.~Nowak} \affiliation{\Lancaster}
\author{N.~Oza} \affiliation{\Columbia}\affiliation{\LANL}
\author{O.~Palamara} \affiliation{\FNAL}
\author{N.~Pallat} \affiliation{\Minnesota}
\author{V.~Paolone} \affiliation{\Pitt}
\author{A.~Papadopoulou} \affiliation{\ANL}
\author{V.~Papavassiliou} \affiliation{\NMSU}
\author{H.~B.~Parkinson} \affiliation{\Edinburgh}
\author{S.~F.~Pate} \affiliation{\NMSU}
\author{N.~Patel} \affiliation{\Lancaster}
\author{Z.~Pavlovic} \affiliation{\FNAL}
\author{E.~Piasetzky} \affiliation{\TelAviv}
\author{I.~D.~Ponce-Pinto} \affiliation{\Chicago}
\author{I.~Pophale} \affiliation{\Lancaster}
\author{X.~Qian} \affiliation{\BNL}
\author{J.~L.~Raaf} \affiliation{\FNAL}
\author{V.~Radeka} \affiliation{\BNL}
\author{A.~Rafique} \affiliation{\ANL}
\author{M.~Reggiani-Guzzo} \affiliation{\Manchester}
\author{L.~Ren} \affiliation{\NMSU}
\author{L.~Rochester} \affiliation{\SLAC}
\author{J.~Rodriguez Rondon} \affiliation{\SDSMT}
\author{M.~Rosenberg} \affiliation{\Tufts}
\author{M.~Ross-Lonergan} \affiliation{\LANL}
\author{C.~Rudolf~von~Rohr} \affiliation{\Bern}
\author{I.~Safa} \affiliation{\Columbia}
\author{G.~Scanavini} \affiliation{\Yale}
\author{D.~W.~Schmitz} \affiliation{\Chicago}
\author{A.~Schukraft} \affiliation{\FNAL}
\author{W.~Seligman} \affiliation{\Columbia}
\author{M.~H.~Shaevitz} \affiliation{\Columbia}
\author{R.~Sharankova} \affiliation{\FNAL}
\author{J.~Shi} \affiliation{\Cambridge}
\author{E.~L.~Snider} \affiliation{\FNAL}
\author{M.~Soderberg} \affiliation{\Syracuse}
\author{S.~S{\"o}ldner-Rembold} \affiliation{\Manchester}
\author{J.~Spitz} \affiliation{\Michigan}
\author{M.~Stancari} \affiliation{\FNAL}
\author{J.~St.~John} \affiliation{\FNAL}
\author{T.~Strauss} \affiliation{\FNAL}
\author{A.~M.~Szelc} \affiliation{\Edinburgh}
\author{W.~Tang} \affiliation{\Tennessee}
\author{N.~Taniuchi} \affiliation{\Cambridge}
\author{K.~Terao} \affiliation{\SLAC}
\author{C.~Thorpe} \affiliation{\Lancaster}\affiliation{\Manchester}
\author{D.~Torbunov} \affiliation{\BNL}
\author{D.~Totani} \affiliation{\UCSB}
\author{M.~Toups} \affiliation{\FNAL}
\author{Y.-T.~Tsai} \affiliation{\SLAC}
\author{J.~Tyler} \affiliation{\KSU}
\author{M.~A.~Uchida} \affiliation{\Cambridge}
\author{T.~Usher} \affiliation{\SLAC}
\author{B.~Viren} \affiliation{\BNL}
\author{M.~Weber} \affiliation{\Bern}
\author{H.~Wei} \affiliation{\Louisiana}
\author{A.~J.~White} \affiliation{\Chicago}
\author{Z.~Williams} \affiliation{\UTA}
\author{S.~Wolbers} \affiliation{\FNAL}
\author{T.~Wongjirad} \affiliation{\Tufts}
\author{M.~Wospakrik} \affiliation{\FNAL}
\author{K.~Wresilo} \affiliation{\Cambridge}
\author{N.~Wright} \affiliation{\MIT}
\author{W.~Wu} \affiliation{\FNAL}
\author{E.~Yandel} \affiliation{\UCSB}
\author{T.~Yang} \affiliation{\FNAL}
\author{L.~E.~Yates} \affiliation{\FNAL}
\author{H.~W.~Yu} \affiliation{\BNL}
\author{G.~P.~Zeller} \affiliation{\FNAL}
\author{J.~Zennamo} \affiliation{\FNAL}
\author{C.~Zhang} \affiliation{\BNL}

\collaboration{The MicroBooNE Collaboration}
\thanks{microboone\_info@fnal.gov}\noaffiliation






==> src/discussion.tex <==
\section{Discussion}




==> src/tikz_preamble.tex <==


\usetikzlibrary{positioning}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{calc}

\definecolor{C1}{HTML}{FFEC94}%E8D0A9}
\definecolor{C2}{HTML}{FFAEAE}%{B7AFA3}
\definecolor{C3}{HTML}{FFF0AA}%{C1DAD6}
\definecolor{C4}{HTML}{B0E57C}%{F5FAFA}
\definecolor{C5}{HTML}{B4D8E7}%{ACD1E9}
\definecolor{C6}{HTML}{56BAEC}%{6D929B}

\colorlet{colorInput}{C1}
\colorlet{colorEventNode}{C1}
\colorlet{colorPreproc}{C5}
\colorlet{colorPredict}{C5}
\colorlet{colorRNN}{C2}
\colorlet{colorOutput}{C6}
\colorlet{colorLegend}{C5}
\colorlet{colorLayer}{C4}
\colorlet{colorBlock}{C1}

